Modified Gravity and Regular Black Hole Models

The prediction of spacetime singularities, regions of infinite curvature where classical physics breaks down, is one of the most profound challenges in General Relativity (GR). In particular, black hole solutions such as the Schwarzschild and Kerr metrics feature central singularities that signal the incompleteness of the theory in high curvature regimes. This thesis is devoted to the study of modified theories of gravity that aim to resolve these singularities and construct physically viable models of regular black holes: black holes that retain an event horizon but exhibit no curvature divergence anywhere in the spacetime ... Throughout the thesis, particular care is taken to ensure that the proposed models are physically sensible: they reduce to GR in the appropriate limits and lead to well behaved curvature scalars. Collectively, these results highlight the viability of regular black hole models in modified gravity theories, providing a promising path toward a consistent semiclassical description of black holes that avoids the need for quantum gravitational resolution of singularities. (Full abstract can be found in document).

==> Chapters/drafts.tex <==





Figure~\ref{fig:charges} illustrates the profiles of these charges. Notably, while the $\mathrm{GF}_1$ charge is monotonic, the $\mathrm{GF}_2$ charge exhibits oscillatory behavior.

\begin{figure}[!hbt]
    \centering
    \vspace{10pt}
    \includegraphics[width=0.7\textwidth]{Figures/plot-q-v1.pdf}
    \caption{Gravitomagnetic charges on a null slice $u = \text{const.}$ of a four-dimensional gyraton, computed in linearized General Relativity and ghost-free theories $\mathrm{GF}_1$ and $\mathrm{GF}_2$, plotted as a function of $\rho/\ell$. All charges are normalized to the General Relativity value $Q_0$.}
    \label{fig:charges}
\end{figure}





\section{Non local physics}

The issues above are also stated sometimes as the ultraviolet (UV) incompleteness of GR since the breakdown of the theory happens at scales associated with UV energies. Furthermore, the theory is known to be perturbatively non-renormalizable \cite{tHooft:1974toh,shomer2007} which is problematic at the quantum level since it means that it cannot be described by a quantum field theory at high energies. In this sense, GR can be understood as an effective field theory working well at low energy. It is known that the problem of renormalization can be ameliorated by introducing higher-order curvature terms into the Einstein-Hilbert action \cite{PhysRevDReno}; for example, a quadratic in curvature action is perturbatively renormalizable in four dimensions. Unfortunately, this theory is pathological since it spawns massive spin 2 unhealthy ghost-like degrees of freedom which break unitarity \cite{quadG}. However, this type of pathology can be avoided if the action contains non-polynomial field derivatives, in other words, a specific class of infinite-derivative operators can prevent the existence of unhealthy ghosts while keeping the renormalizability of the theory \cite{Biswas_2014,tomboulis1997,Modesto_2012}. Interestingly, the presence of such operators also cures the singularities in the theory \cite{Kolar:2023gqi}, as we will see. Since the presence of such non-polynomial differential operators makes the action non-local, these models are known as non-local ghost-free theories \cite{NONLOC, boosNl}. It is our aim in this section to present them.

Our approach will be mainly divided in two parts; we will first discuss the effects of models with conventional operators and the existence of ghost fields, then we will use an infinite derivative scalar field model to illustrate the mechanisms and properties of such models. The features discussed onwards can be generalized to the theory of  non local gravity, it is the aim of this section to highlight them with simplified examples.

\subsection{Local action and ghosts}

We start by considering the following 4-dimensional action for some scalar field $\phi$ in the presence of an external current $J(x)$:

\begin{equation}
S[\phi] = -\int d^4x\left(\frac{a}{2} \phi \Box \phi +\frac{b}{2}m^2\phi^2 - gJ(x)\phi\right) \, .
\end{equation}

Where we leave the two constants $a$ and $b$ arbitrary for now. For the stationary case, the field equation is

\begin{equation}\label{KG}
(a\Delta - bm^2)\phi = gJ \, .
\end{equation}

For a static and spherically symmetric external current of the form $J = J_0\delta^{(3)}(r)$, the solution can be found via the Green’s function method:

\begin{equation}
\phi(r) = gJ_0 \frac{e^{-\sqrt{b/a}mr}}{4a\pi r} \, .
\end{equation}

In the case where $a=b=1$, this is the well-known solution to the screened Poisson equation, associated with the Yukawa potential \cite{Yukawa:1935xg} with important applications in particle physics \cite{Griffiths:2008zz} and which explains nicely why the photon as the force carrier in electromagnetism gives rise to the Coulomb potential due to its zero mass. However, this potential is singular at $r=0$, leading to an infinite force at this location. This problem permeates all of classical physics. It is possible to ameliorate this expression via the inclusion of some additional heavy mass scale $M$, which in turn introduces higher-order derivatives to the field equations. For now, let us introduce such term by hand in equation \ref{KG} for illustration purposes (we consider $a=b=1$):

\begin{equation}
(1 - \frac{\Delta}{M^2})(\Delta - m^2)\phi(r) = gJ_0\delta^{(3)}(r) \quad \to \quad \phi(r) = g J_0\frac{1}{4\pi r}(e^{-mr} - e^{-Mr})\, .
\end{equation}

Notice that this potential is now regular at $r=0$ and that it reproduces the Yukawa potential when $M \to \infty$. Unfortunately, this result is also unphysical as it leads to the emergence of unphysical degrees of freedom known as ghosts, which will be illustrated in the next section.

\subsection{Spooky ghosts}

In this section, we shall consider the case when there is no external current $J(x)=0$. In momentum space, the field equation implies that 

\begin{equation}
a(\omega^2 - \vec{k}^2) = b m^2 \, .
\end{equation}

Which for the choice $a=b$ is nothing but the relativistic dispersion relation $\omega^2 = \vec{k}^2 + m^2 >0$. However, notice that in the $a= -b$ case the above implies that 

\begin{equation}
\omega^2 - \vec{k}^2 = -m^2 >0 \, .
\end{equation}

Which corresponds to the unphysical case of a complex mass. We call scalar fields $\phi$ obeying this relation tachyonic ghost fields. Furthermore, at the quantum level one can show that the propagator of the theory (following the Feynman prescription) is \cite{Zee:2003mt}

\begin{equation}
\Pi_{\mp}(k) = \mp \frac{i}{k^2 + m^2 - i\epsilon} \, .
\end{equation}

Where the minus sign corresponds to the choice $a = b = 1$ and the plus sign corresponds to the choice $a = b = -1$. The $\Pi_{-}(k)$ propagator is healthy since it corresponds to a physical degree of freedom; however, the $\Pi_{+}(k)$ propagator is said to be unhealthy since it violates the optical theorem, which in turn means that unitarity is broken. A scalar field $\phi$ with such a propagator is called a ghost field. Let us emphasize that the presence of these fields is not necessarily bad since they do not always appear as observables of the theory and they are sometimes even necessary for preserving unitarity or are artifacts of gauge fixing.

With the aid of the discussion above, we can define ghosts as fields with negative kinetic energies. For the example in the previous section, the propagator takes the form 

\begin{equation}
\Pi(k) = \frac{i}{(k^2+m^2)(k^2 + M^2)} = -\frac{i}{m^2-M^2}\left( \frac{i}{k^2 + m^2 - i\epsilon} - \frac{i}{k^2 +M^2 - i\epsilon}\right) \, .
\end{equation}

And we can see that the propagator associated with the mass $M$ has the “wrong” sign and therefore it corresponds to an unhealthy ghost.

\section{Non-local action and ghost cleaner}

Non-locality comes as an idea to get rid of a few of the issues we have been commenting on, namely to remove singularities while avoiding the introduction of new degrees of freedom in our theory. Consider the following non-local action 

\begin{equation}
S_{NL}[\phi] = -\frac{1}{2}\int d^4x\left( \phi  f(\Box) \Box\phi + \phi  f(\Box)m^2\phi- 2gJ(x)\phi\right) \, .
\end{equation}

Here the function $f(\Box)$ is known as the “form factor” and it is an entire function of the $\Box$ operator. It is this function that renders the action non-local since we only consider those which can be written as an infinite power series, therefore adding infinitely many derivatives. We demand that they obey $f(0) = 1$ so that we can recover the standard local shape of the action in some limit. That the function be entire means that no zeroes are introduced in the propagator and hence no ghosts are present \cite{modSUpe}, as we will see. The simplest way to show that this mechanism removes singularities is to consider the stationary and massless $m=0$ case where the equations of motion become

\begin{equation}
f(\Delta)\Delta \phi = gJ \, .
\end{equation}

Let us choose a specific example of the form factor which will be broadly used throughout this thesis $f(\Delta) = e^{-\ell^2\Delta}$, here $\ell$ is the scale of non-locality at which the non-local effects become important and has units of length. For a source of the type $J = J_0\delta^{(3)}(r)$, the solution is 

\begin{equation}
\phi(r) =-\frac{gJ_0}{4\pi r}\mathrm{erf}\left(r/2\ell \right) \, .
\end{equation}

Which is now finite at $r= 0$ and furthermore, in the limit where $r \gg2\ell$ one recovers the usual $\phi \sim -1/r$ behavior of the potential. In other words, only as $r$ approaches the scale of non-locality $\ell$ the effects of such non-locality become important while they vanish as this scale becomes negligible. On top of this, let us now look at the propagator of the theory

\begin{equation}
\Pi(k) = \frac{1}{f(-k^2)(k^2+m^2)} \, .
\end{equation}

Because of all of the properties we have imposed to the form factor, there are no new poles in this propagator nor ghost fields, and hence such a propagator is said to be ghost-free. For instance, notice that if the form factor were to be any polynomial $f(-k^2) = \sum_n(-\ell^2k^2)^n$ then 

\begin{equation}
\Pi(k) = \frac{1}{(k^2+m^2)\sum_{n}(-\ell^2k^2)^n} = \frac{1}{k^2+m^2} + \sum_n \frac{a_n}{g_n(-\ell^2k^2)} \, ,
\end{equation}

Where the $a_n$ are constants and the $g_n$ are the irreducible polynomials that factorize the form factor. This propagator introduces as many new fields as the order of $f(-k^2)$. Since $1 + \sum_na_n = 0$ then at least one of the propagators is going to correspond to a ghost field.



In my thesis I am going to discuss the following topics: (1) non local generalizations of the linearized gravity equations and of the Maxwell theory \cite{Boos_2021}; (2) the ultrarelativistic limit of solutions for point like particles in non local models \cite{Boos_2020}; (3) implementing the double image method for searching solutions of the  non-local linearized gravity equations; and (4) non-locality and non singular models of black holes \cite{Frolov:2023jvi}


\jose{OLD APPENDIX ON NON LOCAL}

\chapter{Some Details About Infinite Derivative Gravity}
\label{app:NonLocal}

\section{Potential Regularization}
We will now illustrate the mechanism by which the non-local form factors remove the singularities. Consider equation \ref{Lin_NL} for a point like source $T_{00} = m\delta^{(d)}(\vec{x})$ in $d$ space dimensions, sourced by a potential $\varphi = \varphi(\vec{x})$
\begin{equation}
f(\Delta)\Delta \varphi(\vec{x}) = \frac{\kappa}{2}m\delta^{(d)}(\vec{x}) \, .
\end{equation}
Let us choose the Gaussian form factor $f(\Delta) = e^{-\ell^2\Delta}$. The solution may be found by finding the Green function as
\begin{equation}
    f(\Delta)\Delta G_d(\vec{x},\vec{y}) = \delta^{(3)}(\vec{x} - \vec{y}) \, .
\end{equation}
Then the solution will take the form
\begin{equation}
    \varphi(r) = -2\kappa\frac{d-2}{d-1}m G_d(r) \, .
\end{equation}
Where $r = |\vec{x}|$, $d$ are the spatial dimensions and $G_d$ is the $d$-dimensional Green function which is given by 
\begin{equation}
    G_d(r) = \frac{1}{2\pi} \int_{-\infty}^{\infty} \frac{d\eta}{\eta f(-\eta\ell^2)} \int_{-\infty}^{\infty}d\alpha K_d(r;\alpha)e^{-\eta \alpha} \, .
\end{equation}
and the $d$-dimensional heat kernel, it is given by
\begin{equation}
    K_d(r;p) = \frac{e^{-r^2/4\alpha}}{(4\pi\alpha)^{d/2}} \, .
\end{equation}
Then we can find an explicit solution for the potential, for the explicit case of our form factor in $d=3$ 
\begin{equation}
\varphi(r) =-\frac{\kappa m}{8\pi r}\mathrm{erf}\left(r/2\ell \right) \, .
\end{equation}
Which is finite at $r= 0$ unlike the solution for the local gravitational potential and furthermore, in the limit where $r \gg2\ell$ one recovers the usual $\phi \sim -1/r$ behavior of the potential. In other words, only as $r$ approaches the scale of non-locality $\ell$ the effects of such non-locality become important while they vanish as this scale becomes negligible. This method has been extensively in the literature to for example find a mass gap in black hole formation \cite{Frolov_2015}, the study of ultrarelativistic objects \cite{Frolov_2016, Boos_2020, Boos_2021}, collapse of small masses \cite{frolov2015sphericalcollapsesmallmasses} and much more examples \cite{Giacchini_2019WFL,ScalarKernel,Heredia_2022,Kol__2021,BraneGF}.

There is also an alternative way to go about this, one may rewrite the equation \ref{Lin_NL} as
\begin{equation}
    \Delta\varphi = \frac{\kappa}{2}\rho_{\mathrm{sm}} \, ,
\end{equation}
so that now we have smeared the source and expressed it in terms of the quantity $\rho_{\mathrm{sm}}$ which is given by  $T_{00} = f(\Delta)\rho_{\mathrm{sm}}$. Then, for a point-like particle, it would be given by an effective delta source which can be expressed as 
\begin{equation}
    \rho_{\mathrm{sm}} = \frac{m}{2\pi^2}\int_0^{\infty}dk\frac{k\sin(kr)}{rf(-k^2)} \, .
\end{equation}
Now the solution would be given by 
\begin{equation}
    \varphi(r) = \frac{\kappa}{8\pi}\int_{\infty}^{r}dx\frac{m_{\mathrm{sm}}(x)}{x^2} \, , 
\end{equation}
where $m_{\mathrm{sm}}(r)$ is the effective mass function 
\begin{equation}
    m_{\mathrm{sm}}(r) = 4\pi \int_0^r dx x^2 \rho_{\mathrm{sm}}(x) \, .
\end{equation}
This approach is also used in the literature of local and non-local models. for applications following this approach, see for example, \cite{Burzill__2021,Giacchini_2019,Tseytlin_1995,dePaulaNetto:2023vtg,Buoninfante_2018Ring}.
\section{Propagator}
On top of this, let us now look at the propagator of the theory
\begin{equation}
\Pi(k) = \frac{1}{f(-k^2)(k^2+m^2)} \, .
\end{equation}
Because of all the properties we have imposed to the form factor, there are no new poles in this propagator nor ghost fields, and hence such a propagator is said to be ghost-free. For instance, notice that if the form factor were to be any polynomial $f(-k^2) = \sum_n(-\ell^2k^2)^n$ then 
\begin{equation}
\Pi(k) = \frac{1}{(k^2+m^2)\sum_{n}(-\ell^2k^2)^n} = \frac{1}{k^2+m^2} + \sum_n \frac{a_n}{g_n(-\ell^2k^2)} \, ,
\end{equation}
Where the $a_n$ are constants and the $g_n$ are the irreducible polynomials that factorize the form factor. This propagator introduces as many new fields as the order of $f(-k^2)$. Since $1 + \sum_na_n = 0$ then at least one of the propagators is going to correspond to a ghost field, as we already pointed out in subsection \ref{sec:formfactors}

\section{Initial conditions of non-local equations}



One interesting consequence of working with non-locality as the result of smeared sources in spacetime is the following: for a static source, non-locality results in the spatial smearing of the source. However, for a time dependent source one has to deal with a “time smearing” of the source as well. This may be illustrated by considering a source of the type $J \sim \delta(t - t_0)$, then by using the effective potential approach discussed above one may find (for $N=1$) that

\begin{equation}
J_{\mathrm{eff}} = e^{\ell^2(\Box - m^2)}J \sim e^{-(t-t_0)^2/\ell^2} \, .
\end{equation}

Where we have used the heat Kernel from above to obtain the dependence of the effective source on the last term in the far RHS. Notice that the equations of motion are not indifferent to the spontaneous existence of some external current at $t_0$, in fact, they are affected by it for some time after $t_0$ until this term becomes zero asymptotically. Put in other words, the non-locality makes the effective source linger for some time which in turn alters the dynamics of the system. This is related to the initial value problem of these models which we now address.

One may naturally wonder whether enough initial data can be supplied to the non-local equations of motion to make them predictive as one is after all adding an infinite number of derivatives. It has been shown \cite{NL_InitialCondsandEOM,Barnaby_2008} that there are some instances where this initial value problem is well posed as despite the infinite derivatives, only two pieces of initial data are needed for each pole in the propagator. Basically, nonlocality does not fundamentally change the way initial conditions work. Instead of needing an infinite number of initial conditions, one can reformulate the problem in terms of a local system with the aid of an auxiliary field such that only two initial conditions (typically the value of the field and its first derivative) are necessary to uniquely determine its evolution. This method is known as the diffusion method. As by construction the ghost-free models contain the same number of poles as the local theory the amount of initial data needed is exactly the same. The one caveat is, however, that one must abandon the notion of an infinitely thin $t=\mathrm{constant}$ Cauchy surface in favor of a Cauchy surface with some thickness of the order of the scale of non-locality $\ell$ \cite{Barnaby_2011}.




##############################################################


Through centuries of scientific advancement, we now comprehend that there are fundamental forces in nature whose laws govern the natural phenomena we observe. Notably, gravity dominates on a universal scale. Fully understanding this force is our best shot at unraveling the universe's origin and ultimate fate. Our most comprehensive understanding of gravity is encapsulated in Albert Einstein’s General Relativity theory (GR), expressed mathematically by its field equations \cite{Misner:1973prb}:
\begin{equation}
R_{\mu\nu} - \frac{1}{2}g_{\mu\nu}R + \Lambda g_{\mu\nu} = \frac{8\pi G}{c^4}T_{\mu\nu} \, .
\end{equation}

On the left-hand side, we have the metric tensor $g_{\mu\nu}$, the Ricci tensor $R_{\mu\nu}$, the Ricci scalar $R$, and the cosmological constant $\Lambda$. On the right-hand side, we have the speed of light $c$, Newton’s coupling constant $G$, and the stress-energy tensor $T_{\mu\nu}$. These equations connect the spacetime and its curvature (on the left) with its matter content (on the right). In other words, they describe how matter impacts the surrounding space. The cosmological constant accounts for the expansion of the universe. We will set this constant to zero and choose units where $G=c=1$. Solving these equations involves finding explicit relations that explain the evolution of physical systems. The theory has been successfully applied in predicting phenomena such as gravitational waves and the bending of light, it's also been used to understand structures of the universe like solar systems or galaxy clusters \cite{Will_2018}. However, this theory is still incomplete. A set of phenomena, such as dark matter and the process that gave birth to the universe, remain unexplained by GR \cite{Ryden:1970vsj}.



\section{Exact Solutions of General Relativity}
One of the most surprising discoveries from the theory of GR also revealed one of its greatest mysteries and highlighted its incompleteness. The first solution to Einstein's vacuum field equations was the Schwarzschild metric \cite{schwarzschild1999gravitationalfieldmasspoint}:
\begin{equation}
ds^2 = -\left(1 - \frac{2m}{r} \right)dt^2 + \left(1 - \frac{2m}{r} \right)^{-1}dr^2 + r^2\left(d\theta^2 + \sin^2\theta d\phi^2\right) \, .
\end{equation}

Initially, it wasn't believed to be physically relevant as it described the gravitational field of a spherical mass yet contained unusual features, such as a surface from which nothing, not even light, could escape. It was later realized that such an object could exist due to the gravitational collapse of matter, like dust or a massive star, provided all the matter collapses beyond the Schwarzschild radius $r_S = 2m$ \cite{OppVo, OppSny}. These objects were given the name "black holes". Their existence has been confirmed through both indirect and direct observations, along with the assistance of gravitational wave detectors \cite{CYg1,Cyg2,PhysRevLett.116.061102, PhysRevLett.118.221101, Abbott_2021, M872019}.

A more general and physically realistic case is that of a rotating black hole, described by the Kerr metric \cite{KerrSchild}. The detailed structure and properties of this solution are reviewed in Appendix~\eqref{app:KerrMetric}, and we will not reproduce them here. Nevertheless, it is important to emphasize that the Kerr solution plays a central role in both theoretical and observational aspects of black hole physics. Due to the dynamical nature of astrophysical processes, it is widely expected that most black holes in the universe possess nonzero angular momentum.

Rotation has significant physical consequences. For instance, the spin of a black hole is thought to be a primary driver behind the launching of powerful relativistic jets via mechanisms of energy extraction from the black hole’s rotational energy \cite{EMextractionKerr,BHmodelsAGN}. These jets, in turn, influence star formation rates and the thermal history of the interstellar medium in their host galaxies \cite{Fabian:GalaxyFormation}. Moreover, the inclusion of spin is essential for accurate modeling of accretion disks, which are central to understanding both active galactic nuclei and X-ray binaries \cite{accretionSBH1,accretionSBH2}.

In addition, one of the outstanding puzzles in modern astrophysics is the origin of supermassive black holes (SMBHs) observed at high redshifts \cite{earlySMBH}. Their spin may encode crucial information about the formation mechanisms that produced them—whether through hierarchical mergers, direct collapse, or sustained accretion processes \cite{Spin:SMBH}. Consequently, measuring black hole spin has become a major observational priority \cite{reynolds2019observingblackholesspin}.

From a theoretical perspective, it is essential to understand how rotating black holes interact with their environment. In realistic astrophysical settings, black holes are not isolated, and their interactions with surrounding matter and fields can give rise to a number of important physical effects. These include feedback mechanisms, gravitational wave emission, and possible imprints on the distribution of dark matter and galactic structure. Such phenomena are of particular interest for identifying potential observational signatures; see, for example, \cite{BHingalaxies,Frolov:2024xyo,Frolov:2024tiu,BHinDM} and references therein.


\section{The Need for an Extension of General Relativity}

\subsection{The singularity problem}

There is a crucial aspect of black holes that makes them particularly interesting from a purely theoretical point of view: the singularity. This section aims to explain the significance of this enigmatic region situated beyond the event horizon, at the very core of every black hole, static or rotating. In previous sections, we overlooked the scalar invariants that can be derived from the Kerr metric. Scalar invariants play a pivotal role as mathematical entities that remain invariant under any change of coordinates, offering insights into the spacetime independent of coordinates. While metric equations may exhibit divergences attributable to chosen coordinate systems, which correspond to intriguing regions, interpreting them requires caution as they can be eliminated by suitable coordinate transformations. However, such concerns do not apply to scalar invariants.

Let's delve into the set of scalar invariants known as curvature invariants, encompassing every scalar derivable from the Riemann and Weyl tensors. An exemplary scalar is the Kretschmann invariant $K = R_{\mu\nu\alpha\beta} R^{\mu\nu\alpha\beta}$. For the Schwarzschild metric, it assumes the form:

\begin{equation}\label{KreschSchw}
K = \frac{48 m^2}{r^6}.
\end{equation}

Here lies a pivotal observation: this quantity diverges at the center of the black hole ($r=0$). Now, let's examine this scalar for the Kerr metric:

\begin{equation}
K = \frac{48m^2(r^2-a^2\cos^2\theta)((r^2+a^2\cos^2\theta)^2 - 16r^2a^2\cos^2\theta)}{(r^2 + a^2\cos^2\theta)^6}.
\end{equation}

First, notice that it matches \eqref{KreschSchw} as $a\to0$. However, it diverges at $r=0$ and $\theta = \pi/2$. Remarkably, for a rotating black hole, this divergence occurs on a ring with a radius of $a$. This leads to our initial definition of a curvature singularity: a region where curvature becomes infinite. While several equivalent statements can delineate a singularity, the crux lies in the recognition that such spacetime divergences render the metric and curvature tensor non-differentiable. Consequently, general relativity breaks down, losing its predictive power \cite{Hawking:1976ra}   .

Another precise and mathematical definition of singularities is embodied in the Penrose singularity theorem \cite{Penrose:1964wq,Senovilla:2021pdg, Senovilla:2022vlr}.


\begin{theorem}
In a spacetime exhibiting sufficient differentiability, if:
\begin{itemize}
    \item the null convergence condition holds,
    \item there exists a non-compact Cauchy hypersurface $\Sigma$
    \item and a closed future-trapped hypersurface,
\end{itemize}
then future-incomplete null geodesics exist.
\end{theorem}

We will provide several insights to outline the theorem above, but we'll refrain from delving into all the intricate physical and mathematical concepts, as that's the objective of a more comprehensive review. Essentially, the theorem pertains to the spacetime within a region enclosed by a defined "trapped surface" (see \cite{trapped} for a comprehensible review). We'll illustrate how this framework aptly describes black holes. First, notice that the concept of incomplete null geodesics was introduced, we define them as geodesics lacking an affine parameter extending from $-\infty$ to $\infty$. This leads us to another definition of singularity, one denoting a "failure" of spacetime due to geodesic incompleteness or finite affine parameters. Here, a singularity signifies the "end" of spacetime itself, rather than problematic quantities within it. This definition, although standard, contrasts with our first definition.

For completeness, let's briefly discuss the conditions outlined in the theorem. Null convergence entails satisfying the null energy condition:

\begin{equation}
T_{\mu\nu}\ell^{\mu}\ell^{\nu} \geq 0.
\end{equation}

The presence of a Cauchy hypersurface ensures the existence of a spacelike slice sustaining the initial data, thus completely determining the spacetime. Non-compactness indicates that space is infinite. Lastly, trapped surfaces, introduced by Penrose to characterize the point of no return in gravitational collapse, are closed spacelike surfaces where their area decreases along any possible future direction. Consider a 2D surface $S$, and define the scalar
\begin{equation}
 \kappa = -g^{ab}H_aH_b|_S
\end{equation}
Here, $a$ and $b$ denote coordinates on this surface, and $H_a$ is the mean curvature one form. A surface $S$ is deemed trapped if $\kappa$ is positive; for black hole metrics, the event horizon resides where $\kappa = 0$. This underscores the relevance of the theorem when applied to black holes.

Although our two definitions differ in phrasing, they share a common sentiment: the concept of a singularity poses challenges for general relativity and our understanding of nature. This issue gains special significance, as its resolution is expected to emerge from the fusion of quantum mechanics and general relativity in a theory known as quantum gravity. Quantum gravity becomes imperative in scenarios where both theories must coexist, such as at v ery small distances from the most potent gravitational force in the universe, the center of a black hole. Formulating a consistent theory of quantum gravity is inherently challenging, as it must adhere to the tested behavior of both quantum mechanics and general relativity. Consequently, this thesis focuses on theories aiming to rectify the deficiencies of general relativity at small distances while maintaining its accuracy at large distances, where it's been extensively validated. 


\section{Standard Black Holes vs Regular Black Holes vs Black Hole Mimickers}

To address the singularity problem, it is useful to clarify the terminology and compare different types of black hole solutions. We refer to the solutions of General Relativity that possess both an event horizon and a curvature singularity as \textit{standard black holes}; canonical examples include the Schwarzschild and Kerr metrics. It is important to emphasize that these features are generally regarded as mathematical idealizations, stemming from simplifying assumptions rather than physically realistic descriptions. For instance, the event horizon is not directly observable by any finite-time observer \cite{Horizon:Visser}. Instead, astrophysical black holes are expected to exhibit apparent or trapped horizons, which are physically meaningful observables. Similarly, the singularity is often interpreted as a signal of the breakdown of the classical theory and our ignorance of matter behavior under extreme conditions such as gravitational collapse \cite{crowther2021attitudessingularitiessearchtheory}.

The hope is that these idealizations will be resolved in a more fundamental framework, such as quantum gravity. A promising strategy is to consider modified theories of gravity that alter the short-distance behavior while recovering General Relativity at large distances. These modifications can be interpreted as effective field theories emerging from a more complete quantum gravitational description. This thesis explores such modifications, focusing on constructing black hole solutions with a non-singular core. We refer to these objects as \textit{regular black holes}, and define them by the following criteria:
\begin{itemize}
    \item They possess trapped regions and outer horizons.
    \item They are geodesically complete.
    \item Scalar curvature invariants remain finite at the center, replacing the singularity with a finite core.
\end{itemize}

Closely related to these are \textit{black hole mimickers}, which are horizonless geometries often proposed in alternative theories to address the singularity issue. These are defined as spacetimes that:
\begin{itemize}
    \item Do not contain trapped regions.
    \item May describe ultracompact stars or traversable wormholes.
    \item Have a finite redshift surface, sometimes referred to as the “surface,” which need not be hard.
\end{itemize}

Although this classification is not exhaustive, it captures the essential differences relevant to the models discussed throughout this thesis. For more detailed taxonomies, see \cite{Carballo-Rubio_2020, carballo:geodesicallycompleteBHs}. From a field-theoretic perspective, there are two broad approaches to modifying General Relativity: one can introduce higher-derivative operators acting on curvature tensors, or add higher-order curvature invariants to the action. The former leads to nonlocal ghost-free gravity theories, while the latter gives rise to generalized quasitopological gravities. Both approaches are explored in this work.

\subsection{Some Aspects of Black Hole Mimickers}

We now outline some general features and open problems related to black hole mimickers. One intriguing property is that under matter accretion, these objects may dynamically evolve into standard black holes. Specifically, it has been argued that black hole mimickers can form event horizons once a critical mass is reached, regardless of the underlying microscopic theory \cite{PhysRevD:Carballo_HBH,PhysRevD:Visser_PhenoBH}.

Qualitatively, these objects resemble relativistic stars containing exotic matter beyond the would-be event horizon. Examples include gravastars \cite{pnas:gravasars,Visser:gravastars}, fuzzballs \cite{Mathur:fuzzball,Guo:fuzzball}, and black stars \cite{visser2008kerrspacetimebriefintroduction}. Most models are limited to static or slowly rotating spacetimes, highlighting a central open challenge: the construction of fully rotating mimicker geometries in modified gravity frameworks.

Another unresolved issue is their dynamical formation. In the case of gravastars, recent proposals suggest that they form via a phase transition from a normal matter equation of state to a vacuum-like one with negative pressure. If quantum effects constrain the interior density to be less than the pressure, formation may proceed via the Tolman–Oppenheimer–Volkoff equations \cite{Adler_2025}. Effective action descriptions also exist for the dynamics of mimickers such as boson stars \cite{PRD:bosonstars,PRL:bosonstars} and black shells \cite{PRD:blackshells,PRD:blackshells2}, though these tend to describe low-compactness configurations. Highly compact mimickers remain largely unexplored.

Some proposals suggest that these objects could form from Hawking radiation \cite{KAWI:mimck,Baccetti_2018}, though this remains speculative and debated \cite{Chen:2018,JuarezAubry2018}. Their formation, stability, and interaction with standard matter continue to be active areas of research.

\subsection{Some Aspects of Regular Black Holes}

Regular black holes are typically small deviations from classical black holes, differing only in the innermost region where the singularity is replaced by a regular core. These models are often constructed in a phenomenological manner, without direct derivation from a fundamental theory. Despite the lack of consensus, most regular black hole models share the following properties:
\begin{itemize}
    \item The singularity is replaced by a smooth region with finite curvature invariants, consistent with Markov’s limiting curvature conjecture \cite{limcur_markov}.
    \item A small length scale $\ell_r \ll r_s$ (with $r_s$ the Schwarzschild radius) governs deviations from classical behavior.
    \item The core geometry typically approaches de Sitter space, in line with expectations for high-density matter \cite{Gliner1966}.
    \item The Schwarzschild solution is recovered in the asymptotic limit $r \to \infty$.
    \item The spacetime contains at least two horizons.
\end{itemize}

While these are not strict requirements, they are common to many models in the literature. Notably, recent work has identified classes of theories in which regular black hole solutions can be systematically derived from action principles \cite{QT_BH}.



Another key challenge lies in understanding the formation and evolution of regular black holes. Several works have addressed dynamical formation in quasitopological gravity, including thin-shell collapse \cite{bueno2024,bueno2024shell} and the Oppenheimer–Snyder model \cite{bueno2025oppenheimersnyder}. Energy-dependent couplings inspired by asymptotic safety have also led to regular black hole formation models \cite{PRL:Bonnano}. In 2D dilaton gravity, quantum corrections have been shown to lead to regular collapse outcomes \cite{PRD:Ziprick,PRD:taves}, with potential embeddings in 4D spacetimes. Recent simulations suggest that such models form both trapped and anti-trapped surfaces \cite{Barceló_2015,mdpi:barcelo}, and may lead to unitary evaporation, highlighting their viability as physical black hole alternatives. Dust collapse models in higher order extensions of General Relativity where discussed in \cite{Buoninfante:2024oyi}


\section{Chapter 4 cut content}

We will denote $\vec{r} = (X,Y,Z)$ and $\vec{k} = (k_X,k_Y,k_Z)$, such that
\begin{equation}
    \delta^{(3)}(X,Y,Z) = \frac{1}{(2\pi)^3}\int e^{-i\vec{r}\cdot\vec{k}}d^3\vec{k} \, ,
\end{equation}
and 
\begin{equation}
    G_0(X,Y,Z) = \frac{1}{(2\pi)^3} \int e^{-i\vec{r}\cdot\vec{k}}\tilde{G}_0(k_X,k_Y,k_Z)d^3\vec{k} \, .
\end{equation}
Where $\tilde{G}_0(X,Y,Z)$ is the Fourier transform of the Green function $G_0$. Using equation \eqref{eqreal_Green} we find that
\begin{equation}
    \tilde{G}_0(k_X,k_Y,k_Z) = - \frac{1}{k^2} \, , \quad k^2 = k_X^2 + k_Y^2 + k_Z^2 \, .
\end{equation}
From this equation, we can obtain that
\begin{equation}
    G_0(r) = -\frac{1 }{4 \pi r} \, , \quad r=\sqrt{X^2+Y^2+Z^2} \, .
\end{equation}
This is a result previously derived in chapter \eqref{Ch2}, however, we reproduce it here since we want to highlight the use of the Cartesian coordinates. The function $\Phi$ is 
\begin{equation}
    \Phi(r) = \frac{2M}{r} \, , 
\end{equation}
which, when plugged in equation \eqref{Schw_metric} becomes the Schwarzschild metric in the usual Schwarzschild coordinates.

{\color{blue} {\bf Omit blue!!}
To find a solution for this equation, we have to find an infinite derivative version of the Green function, such that it solves the equation
\begin{equation}
    f(\Delta)\Delta\mathcal{G}(\vec{X}) = \delta^{(3)}(\vec{X}) \, .
\end{equation}
We may write 
\begin{equation}
    \mathcal{G}(X,Y,Z ) = \frac{1}{(2\pi)^3} \int e^{-i\vec{r}\cdot\vec{k}}\tilde{\mathcal{G}}(k_X,k_Y,k_Z)d^3\vec{k} \, .
\end{equation}
And using the same definition for the delta function as above, we find that 
\begin{equation}
    \tilde{\mathcal{G}}(k) = -\frac{1}{f(-k^2)k^2} \, .
\end{equation}
Explicit solutions will of course depend on the explicit form of the form factor $f(\Delta)$, let us consider in particular the choice  
\begin{equation}
    f(\Delta) = \mathrm{exp}\bigg[(-\ell^2\Delta)^N\bigg] \, ,
\end{equation}
where $\ell$, as we know, is the characteristic scale introduced in the infinite derivative models, and therefore it becomes a new parameter which will enter and regularize our black hole solutions.
}

\subsection{Chapter 5 Cut Content}

Consider the metric 
\begin{equation}
    ds^2 - N^2fdt^2 + f^{-1}dr^2+\rho^2d\Omega^2 , ,
\end{equation}
and the reduced action
\begin{equation}
    S = B\int dtdr \mathcal{L} \quad \mathrm{where} \quad \mathcal{L} = \sqrt{-g}L \, .
\end{equation}
We impose on the Lagrangian density to take the form 
\begin{equation}
    \mathcal{L} = -Wh \, ,
\end{equation}
where 
\begin{equation}
    W = \sqrt{-g}\frac{(q-u)}{1-\rho^2p} \, ,
\end{equation}
and the catch is going to be that, now the function $h$ takes the form 
\begin{equation}
    h = h(p,q,u,v) \, .
\end{equation}
It can be checked that the expression for $W$ coincides with \eqref{ASQT} by using the definitions of the basic curvature invariants that can be found in \eqref{app:SphReduction}. We will consider and solve the equations of motion, which are obtained by varying the action
\begin{align}\label{S2D}
    S &= -B\int dt dr Wh \\ 
    &= -B \int dtdr\sqrt{-g}\frac{(q-u)\rho^2}{1-\rho^2p}h(p,q,u,v) \, .
\end{align}
Notice that $h=p$ reproduces the Einstein-Hilbert action, while $h = h(p)$ reproduces the action \eqref{ASQT} from Quasitopological gravity. This means that the action \eqref{S2D} is a generalization of these models. It is important to note that this action is not the result of a symmetry reduction of some higher dimensional covariant action, instead it may be interpreted as an action for a two dimensional non-linear in curvature dilaton gravity, with the dilaton field $\varphi$ given by $\varphi = \ln \rho$. 



FIGURES



\begin{figure}[!hbt]
    \centering
      \includegraphics[width=0.7\textwidth]{Figures/FF7.pdf}
\vspace{-0.5cm}
    \caption{\label{F7}  Plots of $\hat{h}$ (solid line) and $\hat{h}_V(\theta)$ (dash line) as a function of the angle $\theta$ for parameters $\mu=3$ and $\hat{b}=0.3$ ($a=0.9$). }
\end{figure}

\begin{figure}[!hbt]
    \centering
      \includegraphics[width=0.7\textwidth]{Figures/FF8.pdf}
 \vspace{-0.5cm}
   \caption{\label{F8} Plots of $\hat{h}$ (solid line) and $\hat{h}_V(\theta)$ (dash line) as a function of the angle $\theta$ for parameters $\mu=4$ and $\hat{b}=0.3$ ($a=0.9$). }
\end{figure}

\begin{figure}[!hbt]
    \centering
      \includegraphics[width=0.7\textwidth]{Figures/FF9.pdf}
\vspace{-0.5cm}
   \caption{\label{F9} Plots of $\hat{h}$ (solid line) and $\hat{h}_V(\theta)$ (dash line) as a function of the angle $\theta$ for parameters $\mu=3$ and $\hat{b}=0.9$ ($a=0.44$). }
\end{figure}

==> Packages.tex <==
\usepackage{amsthm}
\usepackage{appendix}
\usepackage{euscript}
\usepackage{array}
\usepackage[normalem]{ulem}
\usepackage[hyphens]{url}
\usepackage{lipsum}
\usepackage{xmpincl}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{subcaption}
\usepackage{rotating}
\usepackage{booktabs}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{pdflscape}
\usepackage{textcomp}
\usepackage{longtable}
\usepackage{listings}
\usepackage{pdfpages}
\usepackage{xparse}
\usepackage{ifthen}
\usepackage{hyphenat} 
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage[utf8]{inputenc}
\hypersetup{hidelinks,pdfencoding=unicode,breaklinks=true}
\urlstyle{same}
\Urlmuskip=0mu plus 1mu\relax
\usepackage[
	style=ieee,
	dashed=false,
	doi=false,
	isbn=false,
	url=false,
	citestyle=numeric-comp,
	backend=biber,
	refsegment=chapter,
	sorting=none,
	defernumbers=true]{biblatex}


\newtheorem{theorem}{Theorem}

==> Symbols.tex <==
%Tablularx Additional Column types (c,l,r work as norm)
	%Justified Auto-Width
		%Use a capitial 'X'
	%Centered Auto-Width
		\newcolumntype{C}{>{\centering\arraybackslash}X}
	%Left Justified Auto-Width
		\newcolumntype{L}{>{\raggedright\arraybackslash}X}
	%Right Justified Auto-Width
		\newcolumntype{R}{>{\raggedleft\arraybackslash}X}%

\renewcommand{\arraystretch}{1.5}

\newcommand{\comment}[1]{}%
%Equation Shorthands
	%Non Numbered Equation
		\newcommand{\nonumeq}[1]{\begin{align*}#1\end{align*}}
	%Numbered Equation
		\newcommand{\numeq}[2]{\begin{align}\label{#2}#1\end{align}}
	%Equation Brackets
		\newcommand{\brackS}[1]{\left[#1\right]}
		\newcommand{\brackR}[1]{\left(#1\right)}
		\newcommand{\brackC}[1]{\left{#1\right}}

%Common Symbols
	%Registered Trademark
		\newcommand\regTM{\textsuperscript{\textregistered{}}}
	%Unregistered Trademark
		\newcommand\nonTM{\textsuperscript{\texttrademark{}}}
	%Copyright
		\newcommand\cRight{\textsuperscript{\textcopyright{}}}
	%Copyleft
		\newcommand\cLeft{\textsuperscript{\textcopyleft{}}}
	%Degrees
		\newcommand\degrees{$^\circ$}
    %Hyphen (To allow hyphenation of words with a dash in them)
        \def\hyph{-\penalty0\hskip0pt\relax}
	%Latin
		\newcommand{\latin}[1]{\em#1\em}
	%et al.
		\newcommand\etal{\em et al.\em}
	%etc
		\newcommand\etc{\em etc.\em}
	%e.g.
		\newcommand\eg{\em e.g.\em}
	%i.e.
		\newcommand\ie{\em i.e.\em}
	%Kevlar
		\newcommand\Kevlar{Kevlar\regTM{}}
	%Matlab
		\newcommand\Matlab{\textsc{Matlab}\regTM{}}
